Vulnerability Detection with Fine-grained Interpretations

Despite the successes of machine learning (ML) and deep learning (DL) based vulnerability detectors (VD), they are limited to providing only the decision on whether a given code is vulnerable or not, without details on what part of the code is relevant to the detected vulnerability. We present IVDetect an interpretable vulnerability detector with the philosophy of using Artificial Intelligence (AI) to detect vulnerabilities, while using Intelligence Assistant (IA) via providing VD interpretations in terms of vulnerable statements. For vulnerability detection, we separately consider the vulnerable statements and their surrounding contexts via data and control dependencies. This allows our model better discriminate vulnerable statements than using the mixture of vulnerable code and~contextual code as in existing approaches. In addition to the coarse-grained vulnerability detection result, we leverage interpretable AI to provide users with fine-grained interpretations that include the sub-graph in the Program Dependency Graph (PDG) with the crucial statements that are relevant to the detected vulnerability. Our empirical evaluation on vulnerability databases shows that IVDetect outperforms the existing DL-based approaches by 43%--84% and 105%--255% in top-10 nDCG and MAP ranking scores. IVDetect correctly points out the vulnerable statements relevant to the vulnerability via its interpretation~in 67% of the cases with a top-5 ranked list. It improves over baseline interpretation models by 12.3%--400% and 9%--400% in accuracy.

==> sections/appraoch_retrival.tex <==
\section{CWE Retrieval Model}
\label{cwe:sec}

%If the vulnerability detection section detect that the method $M$ is vulnerable, {\tool} would retrieve the relevant CWEs for the incoming method $M$ to explain why $M$ is vulnerable by using the natural language description. In this section, {\tool} takes the incoming method $M$ as input and providing a list of possible relevant CWEs $CWE_{m}$ with ranking as the output. In order to achieve this, {\tool} uses the Bert \cite{} which has been widely used in neutral language processing problems to deal with it.

If FA-GCN's decision is vulnerable, we also search for the most
closely related CWE for the given method. For this task, we first use
BERT~\cite{BERT} to learn the association between the texts in a CWE and
the vulnerable code in a training dataset of existing
vulnerabilities. For training, in the pre-processing phase, we parse
each statement in the given method into sub-tokens using CamelCase or
Hungarian conventions. We combine all sub-tokens together to get a
sequence of sub-tokens $S_i$ for a statement $i$. For the texts in
CWE, we first connect the title and the description into one
sequence. We then remove stopwords, special characters, and
grammatical words. We also use separators and delimiters as markers,
and zero padding tokens. We then link the CWE sequence and
corresponding vulnerable code sequence as the true labels, and the CWE
sequence and irrelevant code as false labels to train BERT.  In
training, we fine-tune the model by adding a softmax activation layer
on top of the sequence representation vector.

%In {\tool}, in order to retrieve the relevant CWE, we would like to learn the mapping between vulnerable code (only the fixed statements) and their relevant CWEs. So before using Bert to retrieve relevant CWEs for incoming method $M$, we firstly do fine-tuning on the pre-trained Bert model to fit our situation. To do the fine-tuning, in the training data set, we do the following steps:

%\begin{itemize}
%	\item \textbf{Sequence Pre-processing: } As for the vulnerable code, {\tool} break the statements $Stmt_i$ into tokens $T_i$ and for all compound tokens $T_j$, {\tool} breaks them into sub-tokens $ST_j$. By linking all tokens or sub-tokens together, {\tool} gets a sequences $S_i$ that represent the vulnerable statement $Stmt_i$. As for the CWE $k$, {\tool} firstly link the title and the description together as one sequence. And then, {\tool} removes stop words, special characters to also generate a sequence of tokens $S_k$ for the CWE $k$. By using \textit{[CLS]} as the beginning token, \textit{[SEP]} as the separate token, and \textit{[PAD]} as the zero padding token, {\tool} links $S_i$ and the relevant $S_k$ as one sequence which is regarded as the \textit{true label data} for Bert. At the same time, {\tool} links $S_i$ and the irrelevant $S_k$ as one sequence which is regarded as the \textit{false label data}.
%	\item \textbf{Fine-tuning: } As we have pre-processed the data, {\tool} apply them to the Bert to fine-tune the model by adding a \code{Softmax} activation layer on the top of the sequence classification representation vector for the CWE retrieval task.
%\end{itemize}

%Tien
%After training the BERT model, we can use it to find the closest CWE
%to a given code that is detected as vulnerable by our model.

To check if a statement $Stmt$ is relevant to a CWE $D$,
%For a given pair of a statement $Stmt$ and CWE $D$,
we first parse them into sub-tokens and connect into sequences as in
the pre-processing phase of the training. We then use the trained BERT
model on the resulting sequence $S$ of the pair ($Stmt$, $D$). BERT
converts the sub-tokens in the sequence $S$ into the embeddings and
then into the classification representation vector, which is
classified by a softmax function. The score of the function indicates
the relevance degree of $Stmt$ and $D$. We finally add the scores of
all statements in the interpretation sub-graph $G_M$ of a method $M$
to get the relevance score between $M$ and CWE $D$.

 
%After {\tool} has the fine-tuned model for CWE retrieval, we could use it to do the relevant CWE message for incoming method $M$. For each statement $Stmt'_i$ in $M$, {\tool} do the similar step as \textit{Sequence Pre-processing} to generate a sequence $S'_i$ for it. And then, by linking with each CWE together and putting into the Bert, {\tool} could get a list of scores between $[0,1]$ that represent the possibility that the statement $Stmt'_i$ is relevant to each CWE. By adding all scores from all statements in $M$, {\tool} could get the scores that show the possibility that the method $M$ is relevant to each CWE. Base on these scores, {\tool} could retrieve the relevant CWE for the incoming method $M$.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=3.5in]{graphs/Bert.png}
%	\caption{Producing Interpretation Sub-Graphs and Features}
%	\label{fig:cwe}	
%\end{figure} 

%In figure \ref{fig:cwe}, we use \textit{S27} and the \textit{CWE-362} as an example to explain. As you can see in the figure, {\tool} link the sequence of tokens or sub-tokens from the \textit{S27} and the \textit{CWE-362} together by using \textit{[CLS]} as the beginning token, \textit{[SEP]} as the separate token. And then the Bert will automatically transform the input tokens into embedding like \code{E\_{[CLS]}, ..., E\_{m}}. By passing through the network built with transformer models, Bert could generate the final hidden status for each token which you can see as \code{H\_{[CLS]},..., H\_{m}}. To do the statement classification, Bert only pick the first hidden status which is \code{H\_{[CLS]}} as the classification representation vector and then put it into the \textit{Softmax} layer. The final output for the pair of \textit{S27} and \textit{CWE-362} is generated from the \textit{Softmax} and the score shows the possibility if \textit{S27} is relevant to \textit{CWE-362}.


==> sections/cwe.tex <==
\section{CWE Retrieval Model}
\label{cwe:sec}

{\tool} applied a deep learning-based tool Bert \cite{} to learn the
mapping between the keywords $W_{key}$ in existing CWE title and CWE
messages and the relevant vulnerable code $Code_{vul}$. With the
mapping of this, {\tool} can generate some relevant keywords
$W_{key,m}$ for method $m$. By calculating the similarity between each
keyword $W_{key,m,j}$ in $W_{key,m}$ and words in each CWE $k$,
{\tool} can get a similarity score $Score_{m,k}$ for method $M$ and
CWE $k$. With these scores, {\tool} could recommend relevant CWEs for
method $M$ by picking the CWE with highest similarity score.


==> sections/detection.tex <==
\section{Graph-based Vulnerability Detection}
\label{detect:sec}

Taking the incoming method $M$ as input, the first step of {\tool} is
to detect if $M$ is vulnerability or not. In {\tool}, we use a
attention GCN model \cite{} which is a graph-based deep learning model
to classify $M$. In order to make the input suitable for this model,
we generate program dependency graph (PDG) for $M$. To make the node
inside of PDG contains more information about the code, we firstly
braking the statements into sequences as the first feature
$F_{sub-token}$ by only taking variable, method, and class names and
using the CamelCase and Hungarian convention to break each name into a
sequence of sub-tokens. Next, we generate abstract syntax tree (AST)
for $M$ and run a sub-tree summarization tool \cite{} for each
statement to summarize the statements as the second feature
$F_{sub-tree}$. Then, we do statistics on all variables
$V={v_1,...,v_m}$ in method $M$. For each variable $v_i$ in $V$, we
generate a feature $F_{v,i}$ that contains the variable name and the
variable related program slicing $S_i$. The slicing $S_i$ here is
constructed for a single variable $v_i$ which contains all $v_i$
related statements. If one statement does not contains the variable
$v_i$, the relevant feature $F_{v,i}$ will be empty. By combining all
these $m+2$ features for each node in PDG as the node feature set,
attention GCN model can do the whole graph classification for $M$ to
determine if $M$ is vulnerable or not that is the output of this step.


==> sections/discu.tex <==
%\section{Discussion}

==> sections/inter.tex <==
\section{Graph-based Interpretation Model}
\label{interpretation:sec}


==> sections/motiv-overview.tex <==
\subsection{Architecture Overview}


{\tool} has three main modules: vulnerability detection, graph-based
interpretation generation, and natural language-based CWE
retrieval. The input is the source code of a method in a project, and
the output is the detection result and the interpretations.
%If the result is vulnerable, the interpretations include the PDG
%sub-graph, the variables and slices, and the CWE that are relevant to
%the vulnerability. If the result is non-vulnerable, the
%interpretations include the sub-graph and variables, but not CWE.

\subsubsection{Graph-based Vulnerability Detection Model (Section~\ref{detect:sec})}
The input of this model is the source code of the input method $M$ in
a project. Its output is the decision on the vulnerability:
$\mathcal{V}$ or $\mathcal{NV}$, decided via the prediction scores by
our model. The Abstract Syntax Tree (AST) is used to build the vectors
for the statements and the PDG is for the vectors of the method.
%Tien
%{\tool} first parses it to build the abstract syntax tree (AST) and
%program dependence graph (PDG) for $M$. The AST and the code tokens
%are used to build the vector representations for the statements in
%$M$, while the PDG is used to build vector representations for the
%method.
%
For this, we represent the PDG for $M$ with the GCN model~\cite{GCN16}
with an attention mechanism as explained.
%Nodes, edge, and features are used to represent statements,
%dependencies/flows, and program properties.
For training, we use a dataset of pairs of the vulnerable code and
corresponding fixed code, which are labeled accordingly as
$\mathcal{V}$ or $\mathcal{NV}$. For detection, a given method $M$ is
classified by the trained GCN model in a prediction class
and a score.

\subsubsection{Graph-based Interpretation Model (Section~\ref{interpretation:sec})}
%After the GCN model gives the detection result, the graph-based
%interpretation model produces the interpretation.
%
%For this task, we leverage GNNExplainer~\cite{GNNExplainer} that takes
%as input the trained GCN model and the PDG of the give method $M$,
%along with the decision/classification by the GCN ($\mathcal{V}$ or
%$\mathcal{NV}$), to produce two types of interpretations.
%
We use GNNExplainer~\cite{GNNExplainer} that takes as input the
trained GCN model, the PDG of the given method $M$ and the prediction
($\mathcal{V}$ or $\mathcal{NV}$), and produces two types of
interpretations.
%
First, this model produces the sub-graph of the PDG consisting of the
crucial statements that are deemed to be important to classify it as
vulnerable. (For the case of non-vulnerability, the sub-graph can be
considered as the safe statements for the model to decide $M$ as a
safe code). Second, this model produces the list of crucial features,
i.e., the crucial variables and corresponding program slices that are
relevant to the vulnerability.

%
%uses as input the PDG of the input method $M$ and the decision
%($\mathcal{V}$ or $\mathcal{NV}$).
%
%We focus on the class of vulnerability, however, the same mechanism is
%used to produce the interpretation for the non-vulnerability
%class. For clarity, we explain the vulnerability class.xs

%If the detection results show that method $M$ is vulnerable, to explain why our detection model can detect it, we use the explanation model GNNExplainer to generate graph-based explanation for that. Firstly, we regard the vulnerability detection problem as a classification problem and run GNNExplainer to generate a sub-graph $G_{sub}$ from PDG to explain why the attention GCN model provides such result. Next, we use GNNExplainer to analyze the node features used in PDG. The output from GNNExplainer would show that which features are the key features $F_{key}$ that can influence the results from the detection model.
%///

\subsubsection{Natural Language-based CWE Retrieval}
For the given method $M$ that is determined as vulnerable, we perform
an additional step to search for the most related CWE report.  We use
BERT~\cite{BERT}, a neural network model, to learn the association
between the texts in the CWE and the corresponding vulnerable source
code in a training dataset. For a given code, we use the trained model
to produce a list of keywords describing the detected
vulnerable code. We then use the keywords to search for the most
relevant CWE texts.




==> sections/rq1-results-edit.tex <==
\subsubsection{{\bf RQ1. Evaluation on the Interpretations for Vul-detection}}




\begin{table}[t]
	\caption{RQ1. Evaluation on the Interpretations for Vul-detection. The number of edges in a sub-graph is 9.}
	\begin{center}
		\renewcommand{\arraystretch}{1} 
		\begin{tabular}{p{5cm}<{\centering}|p{3cm}<{\centering}}
			\hline
			&  Accuracy \\
			\hline
			Statement Coverage (Vulnerable)             & 73.8\% \\
			
			 Statement Coverage (Non-Vulnerable)           & 67.3\% \\
			\hline
			Variable Coverage Top-5, Top3, Top 1                     & 76.2\%, 46.7\%, 0.093\%\\
			\hline
		Node-Effort                             & 18.9\%\\
			\hline
		Edge-Effort                            & 13.4\%\\
			\hline
		\end{tabular}
		\label{RQ1}
	\end{center}
\end{table}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.25]{graphs/sensitivity-new.png}
	\caption{
		 Sensitivity Analysis: SmallMeth are the percentage of the total number of methods that has smaller size than the sub-graphs as interpretations.}
	\label{fig:RQ1-sen}
	\vspace{-10pt}
\end{figure}

Table~\ref{RQ1} shows that {\tool} can generate the relevant sub-graphs as interpretations for the predictions for the 73.8\% of the vulnerable cases, and the 67.3\% of the non-vulnerable cases. To achieve this high accuracy, only on average 18.9\% of all of the statements in a method need to be inspected (i.e., \code{Node-Effort}) and 13.4\% of the dependency edges in a pdg of a method need to be inspected (i.e., \code{Edge-Effort}). 
Moreover, the top-5 accuracy of variable coverage is 76.2\%, meaning that in the 76.2\% of the cases, the vulnerability relevant variable exists in the top-5 ranked variables. Our top-3 accuracy of variable coverage is 46.7\%, but the top-1 is very low, which indicates that it is very challenging to identify the key variables. 
In the dataset, on average, a method has 15 variables. Thus even we pick 5 variables to study, in 76.2\% of the cases, we do not need to go through another 10 variables for inspection, which can significantly save effort. 
%The statement coverage shows that {\tool} can generate a ISG that can correctly show which statement needs to be changed to fix the vulnerability or by having which statement, the code is no longer to be vulnerable for $71.3\%$ and $64.9\%$ of the vulnerable and non-vulnerable method. The variable coverage percentage shows that {\tool} can provide useful interpretation to cover the key variables that have been used in code changes in $77.4\%$ of all the situations. And the node effort and edge effort shows that, by having the interpretation from {\tool}, developers can save $14.7\%$ and $12.1\%$ effort and time to go through statements and check dependencies on analyzing where is the vulnerability.


For sensitivity analysis, Figure~\ref{fig:RQ1-sen} shows that the blue line indicates that when {\tool} has a greater number of edges, the accuracy of the statement coverage naturally increases, as the number of code statements in a sub-graph as an interpretation increases.  
However, the effort that is required for inspection will increase, as the value of 1-\code{Edge-Effort} decreases (the brown line). 
To train {\tool}, we need to consider the trade-off between the effort and the accuracy. Figure~\ref{fig:RQ1-sen} shows that the blue line and brown line cross each other when the number of edges is about 13, so the average number of nodes is xx, meaning that our generated sub-graphs will be larger in terms of the number of code statements than 33\% of all of the methods in the dataset and our generated sub-graphs as interpretations are not relevant anymore. 

Therefore, in addition to the effort and accuracy, the number of edges in a sub-graph as an interpretation also affect the number of methods that can use our sub-graphs. The yellow line indicates the number of edges increases, the number of smaller methods ratio increase (more methods are smaller compared with our sub-graphs).  
All factors considered, we set the number of edges in a sub-graph to {\bf 9} in {\tool}.  %(the red dash line in Figure~\ref{fig:RQ1-sen}). 

%Also by considering the the smaller methods that cannot be explain well by {\tool} because of the smaller size than the generated sub-graph limitation, the shadow area in figure \ref{fig:RQ1-sen-1} is the actual efficient for {\tool} on different numbers of edges. Based on the situation that when selecting number of edges over 9, the statement coverage increase slower while the smaller methods percentage increase faster. So in order keep the biggest shadow area, {\tool} select 9 as the number of edges.

Figure \ref{fig:RQ1-sen-2} shows that when the variable number over 5, the variable coverage increase slower. 
In order to keep less variables to save developer's effort, {\tool} select 5 as the most suitable variable number.



\begin{figure}[t]
	\centering
	\includegraphics[scale=0.25]{graphs/sensitivity-b-new.png}
	\caption{
		Sensitivity Analysis: The Number of Features}
	\label{fig:RQ1-sen-2}
	\vspace{-10pt}
\end{figure}
		
